OmniShare: Securely Accessing Encrypted Cloud Storage from Multiple Authorized Devices

Cloud storage services like Dropbox and Google Drive are widely used by individuals and businesses. Two attractive features of these services are 1) the automatic synchronization of files between multiple client devices and 2) the possibility to share files with other users. However, privacy of cloud data is a growing concern for both individuals and businesses. Encrypting data on the client-side before uploading it is an effective privacy safeguard, but it requires all client devices to have the decryption key. Current solutions derive these keys solely from user-chosen passwords, which have low entropy and are easily guessed. We present OmniShare, the first scheme to allow client-side encryption with high-entropy keys whilst providing an intuitive key distribution mechanism to enable access from multiple client devices. Instead of passwords, we use low bandwidth uni-directional out-of-band (OOB) channels, such as QR codes, to authenticate new devices. To complement these OOB channels, the cloud storage itself is used as a communication channel between devices in our protocols. We rely on a directory-based key hierarchy with individual file keys to limit the consequences of key compromise and allow efficient sharing of files without requiring re-encryption. OmniShare is open source software and currently available for Android and Windows with other platforms in development. We describe the design and implementation of OmniShare, and explain how we evaluated its security using formal methods, its performance via real-world benchmarks, and its usability through a cognitive walkthrough.

==> contents/background.tex <==
\section{background} 
\label{sec:background}

\subsection{Cloud storage} 
\label{sub:cloudStorage}

Cloud storage is a remote storage service that stores and maintains data
across multiple data centers using cloud-computing technologies. It is a part
of Infrastructure as a Service (Iaas) model of cloud
computing~\cite{csa:cloudSec}. It facilitates its clients to remotely store
data with assurance of high data availabiltiy as well as ability to
synchronize data across multiple devices over the Internet.

\ifsubmission

\else
Two types of cloud storage services are available in the market: One that
offers storage service only to third-party applications via application
programming interfaces (API) e.g. Amazon S3, Rackspace etc. And the other
designed store data of their clients, e.g. Dropbox, Google Drive, OneDrive
etc. In this paper, we only consider cloud storage services that are client
oriented.
\fi

\subsection{Privacy of Client data} 
\label{sub:privacy}

\ifsubmission While outsourcing data, clients also relinquish their control
over data, and rely on the privacy and security mechanism of the cloud storage
for data safekeeping. All major cloud storage providers use secure channels to
protect data in transit from client devices to the storage servers.
Additionally, they encrypt data before storing them on their persistent
storage. Nevertheless, all client data stored on the cloud storage servers are
avaliable in the clear. Anyone with an access to these servers, legitimately
or otherwise, can access and even modify client data without the knowledge of
clients. The storage providers also routinely scan client data and even modify
them to enhance their service offerings~\cite{Ion:HomeisSave}. Ironically,
government agencies also actively collect data from the
Internet~\cite{landau:NSA}. They may even force the cloud storage providers to
allow access to the data without the consent of the data
owner~\cite{soghoian:cloud}.

\else
While outsourcing data, clients also relinquish their control over data, and
rely on the privacy and security mechanism of the cloud storage for data
safekeeping. All major cloud storage providers use secure channels to protect
data in transit from client devices to the storage servers. Additionally, they
encrypt data before storing them on their persistent storage. Nevertheless,
all client data stored on the cloud storage servers are avaliable in the
clear. Anyone with an access to these servers, legitimately or otherwise, can
access and even modify client data without the knowledge of clients. The
storage providers routinely scan client data and even modify them to enhance
their service offerings~\cite{Ion:HomeisSave}.

Ironically, government agencies also actively collect data from the
Internet~\cite{landau:NSA}. They may even force the cloud storage providers to
allow access to the data without the consent of the
data owner~\cite{soghoian:cloud}. The third-party doctrine empowers the
government to access any personal data that is voluntarily shared with third
parties, such as banks, cloud, etc., without direct intervention of the data
owner. In the EU, Data Protection Directive (95/46/EC) requires any entity
receiving personal data from the EU to comply with the EU data protection
rules. Similarly, the Safe Harbor framework regulates the protection of
European data transferred to the US. However, after  the September 11
terror attack, the US approved Patriot Act that enabled the government to
access data stored on the US based company servers regardless of their
physical locations~\cite{whittaker:patriotAct, fraunhofer:cloudSec}.

\fi
An effective way to ensure data privacy is to encrypt data with high-entropy
keys that are controlled by clients before uploading them to the remote
servers. Yet, the cloud providers have hardly any incentive to introduce such
client-specific encryptions~\cite{soghoian:cloud}. Most of the cloud storages
offers subscription for free or at low cost. They also use de-duplication
techniques to reduce the cost of storage where they store only a single copy
of the data regardless of the number of data owners. Some providers even
benefit with the advertisement based revenue model where they regularly scan
client data to display relevant ads~\cite{soghoian:cloud}. Encrypting data
with  client-controlled keys hinders them from benefiting under such business
models.


\subsection{Client-side encyption} 
\label{sub:csencryption}

Clients can nevertheless encrypt their data before outsourcing them to the
cloud to ensure data privacy. A secure method is to encrypt each file with
a separate high-entropy encryption keys that are possibily generated and
protected by secure hardware available on the devices. However, accessing
encrypted files from all client devices requires also requires a mechanism to
distribute the file encyrption keys across the devices.

Commercially available cloud storage solutions like Dropbox, Google Drive,
OneDrive lack options for encrypting files with keys generated at the client
devices. In contrast, solutions like SpiderOak, Wuala, Tresorit and Mega
encrypt each file separately with password-derived encryption keys generated
at the client device before uploading them to their servers. Similarly, tools
like Vivoo, BoxCryptor, Sookasa designed to protect client data in the cloud
storage provide client-side file encryption with the keys generated at the
client devices. These tools integrate with most of the popular cloud storage.
However, they require an additional server to manage and distribute the
encryption keys across client devices. The security of these solutions are
dependent on the strength of the password. 

==> contents/formalanalysis.tex <==
OmniShare protects users' data in cloud storage using a key hierachy beginning with RK. Thus, our key distribution mechanism must protect the secrecy and integrity of RK. The primary goal of our key distribution mechanism can be informally stated as follow. After key distribution, the party who holds the key believe that he handles the key to the correct client. Symmetrically, the client who receives the key believes that he is holding the correct key from the legitimate source. Formally, let A be the new device which does not have the RK to access OmniShare encrypted directory on the cloud storage. B is the previously authorized device. We consider three security properties: implicit/explicit key authentication, and key confirmation that are defined in \cite{menezes1996handbook}. However, the \enquote{key} entity mentioned varies in different cases.

\begin{itemize}
	\item \textbf{Mutual Implicit Root Key authentication:} Assurance for B that A is the only other device that can possibly received RK. Similarly, in the case of A, the property ensures the origin of the received RK so that A cannot be tricked to use a compromised RK. 
	\item \textbf{Implicit SRP Session Key authentication:} In the SRP case, both A and B derive the strong secret Session Key from a low-entropy passcode. The Session Key later on is used to protect RK while transporting RK from B to A. For this reason, we assure that the SRP Session key authentication hold in both case: from B to A and from A to B. Obviously, this is also a condition for RK authentication to hold.
	\item \textbf{SRP Session Key confirmation:} Assurance for B that A is in possession of the correct Session Key and vice versa.
	\item \textbf{Explicit SRP Session Key authentication:} Assurance for B that A is the only other device that is in possession of the correct key and vice versa. The security property hold when both implicit key authentication and key confirmation hold.	
\end{itemize}

In QRP, we achieve impicit key authentication using data origin authentication technique. A's public key is authenticated using its hash value distributed via OOB channel. Thus, RK is protected by an authenticated public key that can only be decrypted by the intended communication partner in the protocol. Subsequently, B's data origin is guaranteed through the use of message authentication code based on the shared secret session key. 

In our SRP key distribution protocol, the session key is formed using a widely recognized authenticated key establishment protocol SRP. Similar to QRP, the established secret session key protect the origin of device B's root key.

In both QRP and SRP, we do not do key confirmation for RK. Firstly, each device manages it own key hierachy. It is important for A to ensure the origin of RK and B to not handle RK to advesaries. However, it is not neccessary for B to confirm that if A has received RK or not. Instead, A will display the result directly to users. Secondly, RK confirmation requires another round of message and possibility other information in previous messages such as B public key. Thus, introducing RK confirmation from A to B increases the protocol running time which has direct impact to the overall user experience. For those reasons, we bypassed key confirmation and explicit key authentication for the RK. \cite{menezes1996handbook} also suggests considering \textbf{Forward secrecy} property when one of the long-term Device Key or RK is compromised. However, since we assume that devices are trusted, we can also bypass \textbf{Forward secrecy} property.

It is worth noting that we have not tried to address other security issues. Errors such as deadlocks,  inappropriate use of cryptosystems or weakness in the cryptosystems itself are not addressed. Practically, we use widely deployed third party libraries Bouncy Castle \cite{bouncycastle} and operating system provided secure APIs namely CNG \cite{cng} and private SharedPreferences \cite{sharedpreferences} for all secure operations.


==> contents/keydistributionfull.tex <==
\section{Key Distribution Protocols}
\label{sec:kdProto}

OmniShare offers two separate key distribution protocols depending on the
device capabilities selected for establishing an OOB channel between the
client devices. The key distribution protocol that includes QR code-based OOB
channel uses the channel to ensure the authenticity and integrity of the
protocol messages exchanged via the cloud storage. Whereas the key
distribution protocol that includes copy and enter OOB channel derives a
shared secret between the devices to secure the key distribution process. The
key distribution protocol uses secure remote password (SRP)
protocol~\cite{rfc2945} to derive a shared session key. The following
subsections explain the two key distribution mechanisms based on the OOB
channel used.

\subsubsection{Key distribution using QR code-based OOB channel}
\label{subsub:keydistQR}

\begin{figure}[th]
   \centering
   \includegraphics[trim=2cm 6cm 8cm 2cm, clip=true, width=1\linewidth]{figs/QRP.pdf}
   \caption{Key distribution protocol message using QR code-based OOB channel}
   \label{fig:keydistQR}
\end{figure}


Figure~\ref{fig:keydistQR} outlines the key distribution protocol that
utilizes QR code-based OOB channel. The new device $A$ delivers its RSA public
key $PK_A$ to the authenticated device $B$ and assures the authenticity of the
public key by displaying the digest $H(PK_A)$ of the key as a QR code.
Additionally, the QR code also includes a nonce $r$ that ensures the integrity
of the message received from the authenticated device via the cloud storage.

The authenticated device captures the QR code using an onboard camera,
extracts the key digest, and the nonce. It then calculates the digest of the
public key of the new device and verifies with the digest received via QR
code. After which it encrypts the root key $RK$ with the public key of the new
device and generates the MAC on the encrypted key $E_{PK_A}$ using the nonce.
The new device receives the encyrpted root key and the MAC, $MAC_r(C)$ via the
cloud storage. The QR code-based OOB channel can be replaced with any other
OOB channel that allows the new device to deliver its public key digest and
the nonce, e.g. using NFC.

\subsubsection{Key distribution using copy and enter OOB channel}
\label{subsub:keydistSRP} 

Figure~\ref{fig:keydistSRP} outlines the key distribution protocol that uses
copy and enter OOB channel to enter a passcode. The protocol is based on SRP
protocol (version 6a) that establishes a secure communication over an
untrusted network by proving the knowledge of the password to the verifier
without revealing the password. OmniShare distributes the root key only once
per device therefore the password used during SRP is a one-time password.
During OOB channel establishment, the new device displays the password as a
6-digit passcode, which the client types into the selected authorized device via
an input keyboard.

\begin{figure}[th]
   \centering
   \includegraphics[trim=1cm 13cm 6cm 2cm, clip=true, width=1\linewidth]{figs/SRP.pdf}
   \caption{Key distribution protocol message using SRP-based OOB channel}
   \label{fig:keydistSRP}
\end{figure}

The SRP is a client-server based protocol where the client authenticates to
the server. In our SRP setup, the new device $A$ takes the role of the SRP client while the selected authorized device $B$ acts as the server. To reduce the
number of message round trips, we slightly modified the message sequence of
the original SRP for the salt value s, yet ensuring the effectiveness of the
protocol. All computations are performed in a finite field $GF(N)$ where $N$
is a constant large prime number. $g$ is a generator in $GF(N)$. The protocol
run as follow:

\begin{enumerate}
    
    \item device $A$ generates random number $a$ and a random string $s$ as a salt. Device $A$ then calculate its client credential $\alpha = g^a$. $\alpha$ and $s$ are sent to device $B$. At the same time, $A$ generates a 6-digits passcode $P$ and displays to client. \eledra{change 'client' to 'user' since client is A} 

    \item Meanwhile, device $B$ chooses a random number $b$. Client \eledra{User} is required to enter the passcode $P$ displayed on device $A$. After receiving the passcode, device $B$ generates its part of the credential $\beta=kv+g^b$ where $k$ and $v$ are chosen based on $N$, $g$ ,$s$ and $P$ as depicted in figure \ref{fig:keydistSRP}. Device $B$ sends $\beta$ back to device $A$. \eledra{beta is server credential, not 'part of'. Credential is to indicate that the one holding it is legit}
    
    \item Both devices then compute the common value $\sigma=g^{(ab+bux)}$. The hash value $K_{ses}$ of $\sigma$ is the cryptographically strong session key. Now, they confirm the session key to complete the protocol. Device $A$ generates confirmation message $M1=H(\alpha,\beta,K_{ses})$ and sends to device $B$.

    \item Since device $B$ has access to $\alpha$, $\beta$ and $K_{ses}$, it calculates it $M1'$ and compares it with the received $M1$. If they match, device $B$ sends the final confirmation value $M2=H(\alpha,M1,K_{ses})$, along with the root key $RK$ which is symmetrically encrypted using $K_{ses}$ to device $A$. A message authentication code $m$ generated with the key $K_{ses}$ is also appended to the message to protect the  integrity of message $m$.

    \item Finally, device $A$ verifies the MAC value $m$ and the confirmation value $M2$. The verification of the values implies that the session key $K_{ses}$ is authenticated. Device $A$ then decrypt the encrypted root key value with $K_{ses}$ to get the root key $RK$
\end{enumerate}

Unlike the original SRP where the server $B$ generates and stores the salt value $s$. In our setup, we do not store anything beforehand on both the devices. Thus, generating $P$ and $s$ from the client side reduces the first message exchange round in the original protocol where the server looks up the client identifier and return $s$. Finally, concatenating the secret $RK$ into the confirmation message $M2$ also saves another extra message round.
